Operator Product Expansion on a Fractal: The Short Chain Expansion for Polymer Networks

We prove to all orders of renormalized perturbative polymer field theory the existence of a short chain expansion applying to polymer solutions of long and short chains. For a general polymer network with long and short chains we show factorization of its partition sum by a short chain factor and a long chain factor in the short chain limit. This corresponds to an expansion for short distance along the fractal perimeter of the polymer chains connecting the vertices and is related to a large mass expansion of field theory. The scaling of the second virial coefficient for bimodal solutions is explained. Our method also applies to the correlations of the multifractal measure of harmonic diffusion onto an absorbing polymer. We give a result for expanding these correlations for short distance along the fractal carrier of the measure.

==> changes <==
%auto-ignore

Changes made to the first submission of cond-mat9604083
All changes are due to an error in eq. (4.10) where a wrong 
'correction' term was removed.

1. Abstract:
Omit the last sentence
>This corrects a blob argument which neglects fractality of the
>carrier itself.

2. Omit two sentences after eq. (1.10):
>As a conclusion we find a correction to the scaling law (1.10).
>This takes into account non trivial scaling properties of the carrier
>of the measure which is the absorbing polymer in this example.

3. Omit last sentence in paragraph after eq.(4.5)
>We will see below, when discussing the multifractal correlations,
>that such a correction has to be introduced in (1.5).

4. In eq. (4.10) omit the 'correction' term
>  -(\gamma-1)/\nu

5. Change two sentences after eq. (4.10)
>Here $ (\gamma-1)/\nu$ is a correction which arises from the
>nontrivial correlations of the polymer, the carrier of the measure
>itself. This could not be seen using mere blob arguments[14].
to
> the relation found by Cates and Deutsch [14].

6. Change the last sentence of the conclusions (IV.D)
>The SCE then gives the answer for short distance correlations on the
>fractal carrier of the measure and introduces a correction to the blob
>result.
to
>The SCE then gives the answer for short distance correlations on the
>fractal carrier of the measure again confirming the blob result.

